Algebraic Test for Asymptotic Stability of Periodic Orbits for Polynomial Systems

We will address the problem of determining the existence and asymptotic stability of a non-trivial periodic orbit in dynamical systems described by polynomial vector fields. To this end, we will lean upon the celebrated results of Borg, Olech and Hartman and newer results of Giesl, who all employ the concept of contraction for this purpose. Importantly, we formulate a numerically tractable algebraic test. The developed algorithm is illustrated in a numerical example.

==> ExLotka3D.tex <==
As an illustrative example of a system with an asymptotically stable
limit cycle, we consider the Lotka-Volterra equations in three
dimensions ($n=3$) given by
\begin{equation}\label{eq:lotka3d}
\begin{split}
\dot{x}=&r_1(1+a-x-az)x\\
\dot{y}=&r_2(x-y)y\\
\dot{z}=&r_3(y-z)z,
\end{split}
\end{equation}
where $r_1,r_2,r_3,a>0$ are constant parameters. The system
\eqref{eq:lotka3d} has the four equilibrium points $(0,0,0)$,
$(1+a,0,0)$, $(1+a,1+a,0)$ and $(1,1,1)$. Furthermore, for the
parameters given in Table \ref{tab:lotkapars}, the system \eqref{eq:lotka3d} is
known to have an asymptotically stable limit cycle
\cite{art:shahruz.01}.

\begin{table}[htbp]
  \centering
  \begin{tabular}{|c|c|}\hline
    $r_1$&2\\\hline
    $r_2$&3\\\hline
    $r_3$&4\\\hline
    $a$&10\\\hline
  \end{tabular}
  \caption{Parameter values for system \eqref{eq:lotka3d} to obtain an asymptotically stable limit cycle.}
  \label{tab:lotkapars}
\end{table}

Figure \ref{fig:lotkatrace} illustrates a trace of the system
\eqref{eq:lotka3d} where the limit cycle is visible.
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\columnwidth]{lotka_plot.eps}
  \caption{A 20 s trace of the system \eqref{eq:lotka3d} using the parameters
    in Table \ref{tab:lotkapars} and an initial condition of
    $(x_0,y_0,z_0)=(2,2,2)$. The equilibria at (0,0,0) and (1,1,1) are
  indicated with an 'x' and the final point at $t$=20 s is indicated
  with a green circle.}
  \label{fig:lotkatrace}
\end{figure}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

